VALHALLA: Visual Hallucination for Machine Translation

Designing better machine translation systems by considering auxiliary inputs such as images has attracted much attention in recent years. While existing methods show promising performance over the conventional text-only translation systems, they typically require paired text and image as input during inference, which limits their applicability to real-world scenarios. In this paper, we introduce a visual hallucination framework, called VALHALLA, which requires only source sentences at inference time and instead uses hallucinated visual representations for multimodal machine translation. In particular, given a source sentence an autoregressive hallucination transformer is used to predict a discrete visual representation from the input text, and the combined text and hallucinated representations are utilized to obtain the target translation. We train the hallucination transformer jointly with the translation transformer using standard backpropagation with cross-entropy losses while being guided by an additional loss that encourages consistency between predictions using either ground-truth or hallucinated visual representations. Extensive experiments on three standard translation datasets with a diverse set of language pairs demonstrate the effectiveness of our approach over both text-only baselines and state-of-the-art methods. Project page: http://www.svcl.ucsd.edu/projects/valhalla.

==> figures/masking.tex <==
\begin{figure*} [h]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=0.45\linewidth]{figures/images/prog_mask_de.pdf} \hfill
        \includegraphics[width=0.45\linewidth]{figures/images/prog_mask_fr.pdf}
        \caption{Evaluation with \textbf{Progressive Masking}.}
        \label{fig:progressive_mask}
     \end{subfigure}
     \qquad
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.45\linewidth]{figures/images/entity_mask_de.pdf} \hfill
         \includegraphics[width=0.45\linewidth]{figures/images/entity_mask_fr.pdf}
         \caption{Evaluation with \textbf{Entity Masking}.}
         \label{fig:entity_mask}
     \end{subfigure}
    % \caption{We plot METEOR scores of \ours and text-only models evaluated on Test2016 split, including relative over baseline.}
    \caption{\textbf{Evaluation under Limited Textual Context}. All results use METEOR scores on Multi30K Test2016 split.}
    \label{fig:masking}
\end{figure*}

==> figures/mmt.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/images/diagram-mmt-cropped.pdf}
    \caption{\todo{Multimodal Machine Translation (MMT) with Discrete Visual Representations.}}
    \label{fig:discrete-mmt}
\end{figure}

==> tables/ablations/external_data.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}[b]{@{}lccccccccc@{}}
\toprule
\textbf{Method} & \textbf{External Data} & \textbf{EN-DE}        & \textbf{EN-ES}     & \textbf{EN-FR}        & \textbf{DE-ES}    & \textbf{ES-FR}        & \textbf{EN-RO} & \textbf{EN-AF} & \textbf{Average}   \\ \midrule
\multirow{2}{*}{\ours}  & & 17.5 ± 0.4   & 27.5 ± 0.2         & 18.8 ± 0.2          & \textbf{11.3 ± 0.2}        & 16.6 ± 0.8          & \textbf{14.4 ± 1.0} & \textbf{14.0 ± 0.5}          & 17.2 ± 0.4 \\
  & \checkmark & \textbf{18.0 ± 0.3}   & \textbf{27.7 ± 0.4}         & \textbf{19.1 ± 0.3}          & \textbf{11.3 ± 0.7}        & \textbf{17.4 ± 0.4}          & 14.1 ± 0.3 & 13.8 ± 0.3          & \textbf{17.3 ± 0.4} \\ \midrule
\multirow{2}{*}{\oursm} &  & 17.4 ± 0.4  & 27.5 ± 0.2  & 18.8 ± 0.2          & \textbf{11.3 ± 0.2}         & 16.6 ± 0.8          & \textbf{14.4 ± 1.0} & \textbf{14.0 ± 0.4}          & 17.2 ± 0.4 \\
  & \checkmark & \textbf{18.0 ± 0.3}   & \textbf{27.8 ± 0.4}         & \textbf{19.1 ± 0.3}          & \textbf{11.3 ± 0.7}        & \textbf{17.4 ± 0.4}          & 13.9 ± 0.4 & 13.9 ± 0.4          & \textbf{17.3 ± 0.4} \\ 
\bottomrule
\end{tabular}}
\caption{Training visual encoder with external data on WIT~\cite{srinivasan2021wit}. \todo{Make inline}}
\label{tab:ablations_external}

==> tables/main/datasets.tex <==
\begin{table*}[ht]
    \centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|cc|ccccccc|cccc}
\Xhline{2\arrayrulewidth}
\textbf{Dataset}          & \multicolumn{2}{c|}{Multi30K~\cite{elliott2016multi30k}}  & \multicolumn{7}{c|}{\multirow{2}{*}{WIT~\cite{srinivasan2021wit}}}  & \multicolumn{4}{c}{WMT2014~\cite{bojar2014findings}}       \\ 
\cline{1-3} \cline{11-14} 
\textbf{Visual Data}      & \multicolumn{2}{c|}{Flickr30K~\cite{young2014image}} & \multicolumn{7}{c|}{}                                                           & \multicolumn{4}{c}{Flickr30K~\cite{young2014image} / WIT~\cite{srinivasan2021wit}}                          \\ \Xhline{2\arrayrulewidth}
\textbf{Source Language}  & EN            & EN            & EN   & EN   & \multicolumn{1}{c|}{EN}   & DE   & \multicolumn{1}{c|}{ES}   & EN         & EN         & EN   & \multicolumn{1}{c|}{EN}  & EN            & EN            \\
\textbf{Target Language}  & DE             & FR            & DE   & ES   & \multicolumn{1}{c|}{FR}   & ES   & \multicolumn{1}{c|}{FR}   & RO         & AF         & DE   & \multicolumn{1}{c|}{FR}  & DE            & FR            \\ \hline
\textbf{\# Train Samples} & 29k            & 29k           & 329k & 287k & \multicolumn{1}{c|}{234k} & 133k & \multicolumn{1}{c|}{122k} & 40k        & 18k        & 3.9m & \multicolumn{1}{c|}{36m} & 100k          & 100k          \\
\textbf{\# Validation Samples} & 1k            & 1k           & 15k & 15k & \multicolumn{1}{c|}{15k} & 10k & \multicolumn{1}{c|}{10k} & 5k        & 5k        & 39k & \multicolumn{1}{c|}{27k} & 39k  & 27k          \\
\textbf{\# Test Samples} & 2.5k            &    2.5k        & 3k & 3k & \multicolumn{1}{c|}{3k} & 2k & \multicolumn{1}{c|}{2k} & 1k        & 1k        & 3k & \multicolumn{1}{c|}{3k} & 3k  &    3k       \\
% \textbf{Vocabulary Size}  & \multicolumn{2}{c|}{10k}       & \multicolumn{5}{c|}{10k}                              & \multicolumn{2}{c|}{2k} & \multicolumn{2}{c|}{40k}        & \multicolumn{2}{c}{10k}       \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{\textbf{Datasets and tasks}. We use $3$ datasets with total $13$ tasks that covers various languages with different scales of training data.}
    \label{tab:datasets}
\end{table*}

==> tables/main/wit_with_meteor.tex <==
\begin{table*}[ht]
\small
\centering


\begin{subtable} [b] {\linewidth}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}l|ccc|cc|cc|c@{}}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Well-Resourced}}    & \multicolumn{2}{c|}{\textbf{Non-English}}  & \multicolumn{2}{c|}{\textbf{Under-Resourced}} & \multirow{2}{*}{\textbf{Average}}    \\
\cline{2-8} 
 & \textbf{EN $\rightarrow$ DE}        & \textbf{EN $\rightarrow$ ES}     & \textbf{EN $\rightarrow$ FR}        & \textbf{DE $\rightarrow$ ES}    & \textbf{ES $\rightarrow$ FR}        & \textbf{EN $\rightarrow$ RO} & \textbf{EN $\rightarrow$ AF} &    \\ \Xhline{2\arrayrulewidth}
Text-Only   & 16.0 ± 0.5          & 24.8 ± 0.8          & 16.1 ± 1.2    & 10.7 ± 0.2  & 16.2 ± 0.3  & 11.5 ± 0.7 & 10.8 ± 0.6   & 15.1 ± 0.6 \\
UVR-NMT~\cite{zhang2020neural}     &           &           &           &          &           &  &           &  \\ 
RMMT~\cite{wu2021good}    &           &          &          &           &          &  &          &  \\
Gated Fusion~\cite{wu2021good}        &           &          &          &           &          &  &          &  \\
\ours   & 17.5 ± 0.4   & 27.5 ± 0.2         & 18.8 ± 0.2          & 11.3 ± 0.2        & 16.6 ± 0.8          & 14.4 ± 1.0 & 14.0 ± 0.5          & 17.2 ± 0.4 \\
\oursm  & 17.4 ± 0.4  & 27.5 ± 0.2  & 18.8 ± 0.2          & 11.3 ± 0.2         & 16.6 ± 0.8          & 14.4 ± 1.0 & 14.0 ± 0.4          & 17.2 ± 0.4 \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\vspace{-1mm}
\caption{BLEU score}
\end{subtable} \\[2mm]

\begin{subtable} [b] {\linewidth}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}l|ccc|cc|cc|c@{}}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Well-Resourced}}    & \multicolumn{2}{c|}{\textbf{Non-English}}  & \multicolumn{2}{c|}{\textbf{Under-Resourced}} & \multirow{2}{*}{\textbf{Average}}    \\
\cline{2-8} 
 & \textbf{EN $\rightarrow$ DE}        & \textbf{EN $\rightarrow$ ES}     & \textbf{EN $\rightarrow$ FR}        & \textbf{DE $\rightarrow$ ES}    & \textbf{ES $\rightarrow$ FR}        & \textbf{EN $\rightarrow$ RO} & \textbf{EN $\rightarrow$ AF} &    \\ \Xhline{2\arrayrulewidth}
Text-Only   & 35.4 ± 0.5          & 44.6 ± 1.7          & 37.4 ± 1.3    & 33.3 ± 0.3  & 37.0 ± 0.2  & 26.6 ± 0.6 & 30.2 ± 1.0   & 34.9 ± 0.8  \\
UVR-NMT~\cite{zhang2020neural}     &           &           &           &          &           &  &           &  \\ 
RMMT~\cite{wu2021good}    &           &          &          &           &          &  &          &  \\
Gated Fusion~\cite{wu2021good}        &           &          &          &           &          &  &          &  \\
\ours   & 36.8 ± 0.5   & 47.1 ± 0.2         & 40.2 ± 0.3          & 34.3 ± 0.3        & 37.5 ± 0.9          & 30.4 ± 0.9 & 34.2 ± 0.2          &  37.2 ± 0.5  \\
\oursm  & 36.7 ± 0.5  & 47.1 ± 0.3  & 40.2 ± 0.3          & 34.3 ± 0.4         & 37.5 ± 0.9          & 30.5 ± 0.9 & 34.2 ± 0.2          & 37.2 ± 0.5 \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\vspace{-1mm}
\caption{METEOR score}
\end{subtable}

\caption{\small{\textbf{Machine Translation Results on WIT~\cite{srinivasan2021wit}}.} \todo{mark baselines as reimplemented}}
\label{tab:wit}
\end{table*}
